MusicLM: Generating Music From Text

We introduce MusicLM, a model generating high-fidelity music from text descriptions such as "a calming violin melody backed by a distorted guitar riff". MusicLM casts the process of conditional music generation as a hierarchical sequence-to-sequence modeling task, and it generates music at 24 kHz that remains consistent over several minutes. Our experiments show that MusicLM outperforms previous systems both in audio quality and adherence to the text description. Moreover, we demonstrate that MusicLM can be conditioned on both text and a melody in that it can transform whistled and hummed melodies according to the style described in a text caption. To support future research, we publicly release MusicCaps, a dataset composed of 5.5k music-text pairs, with rich text descriptions provided by human experts.

==> removed.tex <==
\paragraph{Training directly on music-text pairs.}
\label{results/music-text}
Not all text-conditioned generative models rely of joint modality embedding models such as CLIP~\cite{clip} or {\mulan}. Instead, they consume text representations extracted from a text-only language model and learn to  generate audio conditioning on such representations~\citep{parti, audiogen}. Hence, we experiment with a similar setting, making use of a T5X based text encoder~\cite{t5} pre-trained on a large corpus of text-only data. We use an encoder model which has the same size as the {\mulan} text embedding network and predict both semantic tokens and coarse acoustic tokens in a single stage. We evaluate 3 variants of encoder-decoder models by (1) keeping the encoder frozen, (2) finetuning the pre-trained encoder, and (3) training both encoder and decoder from scratch. We train the models on the music-text MuLan training data. We compare to a variation of our approach trained on the audio only part of the MuLan training data.
As we can see from the KLD and MCC scores shown in \cref{table:text2music}, neither of the approaches trained directly from the noisy MuLan training data performs better than our base model on the evaluation set.
We believe such results are the consequence of the weak association between music-text pairs. Hence, we expect this could be tackled by improving the training data, or exploiting a stronger pre-trained text encoder.

\begin{table}[]
\caption{Training directly on noisy $\langle$music, text$\rangle$ pairs using an encoder-decoder architecture, compared to using the pre-trained model MuLan.}
\label{table:text2music}
\vskip 0.15in
\begin{center}
\scriptsize
\begin{sc}
\begin{tabular}{lcccc}
\toprule
Model & FAD$_{\text{Trill}}$ $\downarrow$ & KLD $\downarrow$ & MCC $\uparrow$ \\
\midrule
Base & 0.41 & 3.83$\cdot10^{-04}$ & 0.51 \\
Frozen encoder & 0.42 & 5.48$\cdot10^{-04}$ & 0.30 \\
From scratch & 0.40 & 5.37$\cdot10^{-04}$ & 0.32 \\
Finetuned & 0.43 & 5.45$\cdot10^{-04}$ & 0.30 \\
\bottomrule
\end{tabular}
\end{sc}
\end{center}
\vskip -0.1in
\end{table}


\paragraph{Levels of MuLan RVQ quantizer.}
We investigate the amount of information carried by different RVQ levels of the MuLan quantizer. We train both the semantic and acoustic modeling stage using 12, 6, and 1 RVQ levels. We evaluate different combinations of these stages in \cref{table:mulan-rvq}. Unsurprisingly, general audio quality, as measured by the FAD metric, is not affected by way the text conditioning is encoded. Instead, the adherence of the generated music to the text description, as measured by KLD and MCC metrics, rapidly decreases by conditioning on fewer RVQ levels. Based on these observations we can conclude that (1) the conditioning signal is contained within all levels of the RVQ and (2) using the most fine-grained level of MuLan conditioning (12 RVQ layers to condition both stages) achieves the best results.

\begin{table}[ht]
\caption{Using different combination of MuLan RVQ levels used in the semantic and acoustic modeling stages. While the FAD metric is comparable across models, the adherence to the text description decreases sharply by conditioning on fewer MuLan tokens, as measured by the KLD and MCC metrics.}
\label{table:mulan-rvq}
\vskip 0.15in
\begin{center}
\scriptsize
\begin{sc}
\begin{tabular}{lcccc}
\toprule
Stage$_1$ & Stage$_2$ & FAD$_{\text{Trill}}$ $\downarrow$ & KLD $\downarrow$ & MCC $\uparrow$ \\
\midrule
12 & 12 & 0.43 & 3.78$\cdot10^{-04}$ & 0.51 \\
6 & 12 & 0.43 & 4.02$\cdot10^{-04}$ & 0.49 \\
12 & 6 & 0.43 & 4.08$\cdot10^{-04}$ & 0.48 \\
6 & 6 & 0.43 & 4.18$\cdot10^{-04}$ & 0.47 \\
1 & 12 & 0.42 & 4.24$\cdot10^{-04}$ & 0.46 \\
12 & 1 & 0.44 & 4.26$\cdot10^{-04}$ & 0.45 \\
1 & 1 & 0.43 & 4.83$\cdot10^{-04}$ & 0.37 \\
\bottomrule
\end{tabular}
\end{sc}
\end{center}
\vskip -0.1in
\end{table}

